Subquadratic Algorithms for Algebraic Generalizations of 3SUM

The 3SUM problem asks if an input $n$-set of real numbers contains a triple whose sum is zero. We consider the 3POL problem, a natural generalization of 3SUM where we replace the sum function by a constant-degree polynomial in three variables. The motivations are threefold. Raz, Sharir, and de Zeeuw gave a $O(n^{11/6})$ upper bound on the number of solutions of trivariate polynomial equations when the solutions are taken from the cartesian product of three $n$-sets of real numbers. We give algorithms for the corresponding problem of counting such solutions. Gr\o nlund and Pettie recently designed subquadratic algorithms for 3SUM. We generalize their results to 3POL. Finally, we shed light on the General Position Testing (GPT) problem: "Given $n$ points in the plane, do three of them lie on a line?", a key problem in computational geometry. We prove that there exist bounded-degree algebraic decision trees of depth $O(n^{\frac{12}{7}+\varepsilon})$ that solve 3POL, and that 3POL can be solved in $O(n^2 {(\log \log n)}^\frac{3}{2} / {(\log n)}^\frac{1}{2})$ time in the real-RAM model. Among the possible applications of those results, we show how to solve GPT in subquadratic time when the input points lie on $o({(\log n)}^\frac{1}{6}/{(\log \log n)}^\frac{1}{2})$ constant-degree polynomial curves. This constitutes a first step towards closing the major open question of whether GPT can be solved in subquadratic time. To obtain these results, we generalize important tools --- such as batch range searching and dominance reporting --- to a polynomial setting. We expect these new tools to be useful in other applications.

==> sec/03-algorithms/00-intro.tex <==
\section{Algorithms}
\label{sec:algorithms}

%We now present new algorithms to solve polynomial generalizations of
%3SUM in subquadratic time. We first explore the case where, instead of
%determining whether any triple of input numbers sums to zero, we want to
%decide, for a fixed bivariate polynomial function $f \in \mathbb{R}[x,y]$ of
%constant degree, whether there exists any triple $(a,b,c)$ of input numbers
%such that $c = f(a,b)$. This first problem is called \emph{explicit 3POL}.
%We then generalize the 3SUM problem even more: we want to
%decide, for a fixed trivariate polynomial function $F \in \mathbb{R}[x,y,z]$
%of constant degree, whether there exists any triple $(a,b,c)$ of input numbers
%such that $F(a,b,c)=0$. This second problem is called \emph{3POL}.

We look at both uniform and nonuniform algorithms for explicit 3POL and 3POL\@.
We begin with an $O(n^{\frac{12}{7}+\varepsilon})$-depth algebraic computation
tree for explicit 3POL.
%
We continue by giving a similar real-RAM algorithm for explicit 3POL that
achieves subquadratic running time.
%
Then we go back to the bounded-degree ADT for explicit 3POL and
generalize it to work for 3POL.
%
Finally, we give a similar real-RAM algorithm for 3POL that runs in
subquadratic time.
%%
%\remark{We should also explain why our algorithm
%has a smaller bound than the combinatorial bound, even though it can
%list out all solutions (in concise form).}

